LNS-Madam: Low-Precision Training in Logarithmic Number System using Multiplicative Weight Update

Representing deep neural networks (DNNs) in low-precision is a promising approach to enable efficient acceleration and memory reduction. Previous methods that train DNNs in low-precision typically keep a copy of weights in high-precision during the weight updates. Directly training with low-precision weights leads to accuracy degradation due to complex interactions between the low-precision number systems and the learning algorithms. To address this issue, we develop a co-designed low-precision training framework, termed LNS-Madam, in which we jointly design a logarithmic number system (LNS) and a multiplicative weight update algorithm (Madam). We prove that LNS-Madam results in low quantization error during weight updates, leading to stable performance even if the precision is limited. We further propose a hardware design of LNS-Madam that resolves practical challenges in implementing an efficient datapath for LNS computations. Our implementation effectively reduces energy overhead incurred by LNS-to-integer conversion and partial sum accumulation. Experimental results show that LNS-Madam achieves comparable accuracy to full-precision counterparts with only 8 bits on popular computer vision and natural language tasks. Compared to FP32 and FP8, LNS-Madam reduces the energy consumption by over 90% and 55%, respectively.

==> algorithm/LNS-madam.tex <==
% \setlength{\textfloatsep}{0.5pt}
% \begin{wrapfigure}{R}{0.5\textwidth}
% % \vspace{-23pt}
%     \begin{minipage}{0.5\textwidth}
%         \begin{algorithm}[H]
%         \caption{
%             \textit{LNS-Madam}
%         }
%         % \algnewcommand\algorithmicinput{\textbf{Initialise:}}
%         % \algnewcommand\Initialise{\item[\algorithmicinput]}
        
%         \begin{algorithmic}
%         \STATE {\bfseries Require:} Base-2 weight exponents $\Tilde{W}$, where $\Tilde{W}=\log_2(W)$, learning rate $\eta$, momentum $\beta$
        
%         \STATE Initialize $g_{2} \gets 0$
%         %                 \Comment{initialise first and second moment estimates}
%         \REPEAT
%         \STATE $g\gets \mathrm{StochasticGradient()}$ 
%         %                 \Comment{collect gradient}
%         % \Comment{update first moment estimate}
%         \STATE $g_{2} \gets (1-\beta) g^2 + \beta g_{2}$                        
%         % \Comment{update second moment estimate}
%         \STATE $g^{*} \gets g/\sqrt{g_{2}} $
%         % \Comment{round regularized gradient into integer}
        
%         \STATE $\Tilde{W} \gets \Tilde{W} -\, \eta\, g^{*} \odot sign(W)$
%         %                 \Comment{update weights on their logarithmic scale}
        
%         \UNTIL{converged}
%         \end{algorithmic}
%         \label{alg:lns_madam}
%         \end{algorithm}
%     \end{minipage}
% % \vspace{-25pt}
% \end{wrapfigure}

% \vskip -0.13in
\begin{algorithm}[t]
\caption{
    \textit{Madam optimizer on LNS}
}
% \algnewcommand\algorithmicinput{\textbf{Initialise:}}
% \algnewcommand\Initialise{\item[\algorithmicinput]}

\begin{algorithmic}
\STATE {\bfseries Require:} Base-2 weight exponents $\Tilde{W}$, where $\Tilde{W}=\log_2(W)$, learning rate $\eta$, momentum $\beta$

\STATE Initialize $g_{2} \gets 0$
%                 \Comment{initialise first and second moment estimates}
\REPEAT
\STATE $g\gets \mathrm{StochasticGradient()}$ 
%                 \Comment{collect gradient}
% \Comment{update first moment estimate}
\STATE $g_{2} \gets (1-\beta) g^2 + \beta g_{2}$                        
% \Comment{update second moment estimate}
\STATE $g^{*} \gets g/\sqrt{g_{2}} $
% \Comment{round regularized gradient into integer}

\STATE $\Tilde{W} \gets \Tilde{W} -\, \eta\, g^{*} \odot sign(W)$
%                 \Comment{update weights on their logarithmic scale}

\UNTIL{converged}
\end{algorithmic}
\label{alg:lns_madam}
\end{algorithm}

==> algorithm/quant_madam.tex <==
\begin{algorithm}[H]
\caption{
    \textit{Madam}---a multiplicative adaptive moments based optimizer from \cite{bernstein2020learning}.
}
  
\algnewcommand\algorithmicinput{\textbf{Initialise:}}
\algnewcommand\Initialise{\item[\algorithmicinput]}

\begin{algorithmic}
\item[\textbf{Optimization parameters:}]
    learning rate $\eta$;
    averaging constant $\beta$;
    weight clipping $\sigma^*$.
\State $\bar{g} \gets 0$
\Repeat
    \State $g\gets \mathrm{StochasticGradient()}$ 
    \State $\bar{g}^2 \gets (1-\beta) g^2 + \beta \bar{g}^2$                    
    \State $W \gets W \odot \exp [-\eta \, \sign (W) \odot \clamp(g/\bar{g})]$
    \State $W \gets \clamp_{\sigma^*} (W)$
\Until{converged}
\end{algorithmic}
\label{alg:madam}
\end{algorithm}

==> figures/approximation.tex <==
\begin{figure*}[t!]
    \label{fig:qaa_imagenet}
    \vskip 0.2in
    \centering
    \includegraphics[scale=0.4]{icml2021_submission/figures/approximation.pdf}
    \vskip -0.2in
    \caption{Benchmarking the conversion approximation. \textbf{Placeholder}}
\end{figure*}

==> figures/bfloat16.tex <==
\usetikzlibrary{decorations.pathreplacing}

\begin{center}

\scalebox{0.75}{
\begin{tikzpicture}
    [box/.style={rectangle,draw=black,thick, minimum size=0.6cm}]
\node(sign)[box,fill=black,text=white]  at (0.0,0){S};
\foreach \x in {1,2,...,12}{
    \node[box,fill=gray] at (\x/1.666,0){E};
}
\node[below of =  sign, yshift = 0.0
cm](signlabel){1-bit sign};
\draw[latex-] (sign) to[out=-90,in=90,looseness=1.8] (signlabel);
\draw [thick, black,decorate,decoration={brace,amplitude=10pt,mirror}](0.4,-0.4) -- (7.4,-0.4) node[black,midway,yshift=-0.6cm] {12-bit exponent};
\end{tikzpicture}
}

\end{center}

==> sections/10-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See section \ref{sec:experiments}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See section \ref{sec:quantized_weight_update}}
	\item Did you include complete proofs of all theoretical results?
	% Needs to include in the appendix
    \answerYes{See appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  % Needs to include in the appendix
    \answerYes{See both section \ref{sec:experiments} and appendix}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  % Needs to include in the appendix
    \answerYes{See both section \ref{sec:experiments} and appendix}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
	% Needs to include in the appendix
    \answerYes{See appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  % Needs to include in the appendix
    \answerYes{}
  \item Did you mention the license of the assets?
  % Needs to include in the appendix
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  % Needs to include in the appendix
    \answerYes{See appendix}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  % Needs to include in the appendix
    \answerYes{See appendix}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/11-ack.tex <==
\section*{Acknowledgements}

We would like to sincerely thank Mohammad Shoeybi and Yuanyuan Shi for meaningful discussions and suggestions. A. Anandkumar gratefully acknowledges the support from Bren endowed chair at Caltech.

==> sections/x-energy.tex <==
% \section{Energy Estimation for LNS}



==> tables/5-forward-8-backward-results.tex <==
\begin{table*}[t!]
    \caption{\small{Benchmarking multi-base LNS on various datasets and models. We compare multi-base LNS with INT and FP32 baselines. A unified bitwidth setting is used across tasks: 5-bit for activation gradients $\equant$, and 8-bit for weights $\wquant$, activations $\aquant$ and weight gradients $\gquant$. Each task uses a uniform number of training epochs. Energy reduction compares both the absolute and relative training costs between LNS and FP32 (the higher the better).}}
    \centering
    %     \emph{Note: all Madam runs use initial learning rate $\mathit{\eta=0.01}$.\\
    %  For all algorithms, $\mathit{\eta}$ is decayed by 10 when the loss plateaus.} 
    
    % \vspace{0.5em}
    \tabcolsep=0.15cm
    \small
        \begin{tabular}{cccccc}
        \toprule
        \textbf{Dataset} & 
        \textbf{Task} &
        \textbf{Multi-Base LNS} &
        \textbf{INT} &
        \textbf{Full-Precision} &
        \textbf{Energy Reduction}
        \\
        % \begin{tabular}{@{}c@{}}\textbf{Fixed-Point}\\\textbf{Quantization}\end{tabular} &
        % \begin{tabular}{@{}c@{}}\textbf{Full-Precision}\\\textbf{Baseline}\end{tabular} \\
        \midrule
        % CIFAR-10  & Resnet18 & SGD  & 0.1 & $91.8\pm1.3$ & 0.01 & $92.2\pm0.2$ \\
        CIFAR-10  & ResNet-18   & $93.37\% \pm 0.17$ & $93.28\% \pm 0.15$ & $93.51\% \pm 0.23$ & \num{2.7e-3} KWh (98.4\%) \\
        ImageNet  & ResNet-50   & $75.89\% \pm 0.05$ & $73.82\% \pm 0.06$ & $76.38\% \pm 0.05$ & \num{5.7e-1} KWh (98.4\%) \\
        SQuAD     & BERT-base   & $87.90\% \pm 0.21$ & $23.7 \% \pm 0.49$ & $88.36\% \pm 0.19$ & \num{6.8e-3} KWh (98.3\%) \\
        SQuAD     & BERT-large  & $90.34\% \pm 0.17$ & $16.1 \% \pm 0.62$ & $90.80\% \pm 0.22$ & \num{2.4e-2} KWh (98.3\%) \\
        GLUE      & BERT-base   & $88.07\% \pm 0.45$ & $81.03\% \pm 0.32$ & $88.92\% \pm 0.39$ & \num{4.2e-4} KWh (98.3\%) \\
        GLUE      & BERT-large  & $89.15\% \pm 0.41$ & $87.87\% \pm 0.36$ & $89.35\% \pm 0.44$ & \num{1.5e-3} KWh (98.3\%) \\
        %specifically, ResNet-50 use BF=16 and others use BF=8
        \bottomrule
        \end{tabular}
        \label{tab:standard_benchmark}
        % \vskip -0.2in
    \end{table*}

==> tables/approximation_results.tex <==
\begin{table}[h!]
  \centering
\begin{tabular}{lccc}
    \toprule
     & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    \textbf{$\gamma=4,b_m=0$} & 80.2 & 80.8 & 87.1 \\
    \textbf{$\gamma=4,b_m=1$} & 80.9 & 81.2 & 85.4 \\
    \textbf{$\gamma=4,b_m=2$} & 80.3 & 80.1 & 87.8 \\
    \bottomrule
    
  \end{tabular}
  \caption{Benchmarking hybrid addition approximation on GLUE MPRC task.  }
  \label{tab:approximation_glue}
\end{table}

\begin{table}[h!]
  \centering
\begin{tabular}{lccc}
    \toprule
     & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    \textbf{$\gamma=4,b_m=0$} &  &  & 86.9 \\
    \textbf{$\gamma=4,b_m=1$} &  &  & 87.0 \\
    \textbf{$\gamma=4,b_m=2$} &  &  & 87.9 \\
    \bottomrule
    
  \end{tabular}
  \caption{Benchmarking hybrid addition approximation on SQUAD. F1 scores are provided.}
  \label{tab:approximation_squad}
\end{table}

\begin{table}[h!]
  \centering
\begin{tabular}{lccc}
    \toprule
     & 
    \textbf{Test Accuracy} \\
    \midrule
    \textbf{$\gamma=16,b_m=0$} &  \\
    \textbf{$\gamma=16,b_m=1$} &  \\
    \textbf{$\gamma=16,b_m=2$} &  \\
    \textbf{$\gamma=16,b_m=3$} &  \\
    \textbf{$\gamma=16,b_m=4$} &  \\
    \bottomrule
    
  \end{tabular}
  \caption{Benchmarking hybrid addition approximation on ImageNet with 8 bits weight and activation.}
  \label{tab:approximation_imagenet}
\end{table}

==> tables/best_combination.tex <==


\begin{table}[H]
\caption{\small{A list of appropriate combinations of bitwidth $\bitwidth$ and base factor $\gamma$ given a fixed log dynamic range (0,32).}}
\centering
\small
    \begin{tabular}{cc}
    \toprule
    \textbf{Bitwidth $\bitwidth$} & \textbf{Base Factor $\gamma$}
    \\
    \midrule
        \textbf{8-bit
    } &  8    \\
        \textbf{7-bit
    } &  4    \\
        \textbf{6-bit
    } &  2    \\
        \textbf{5-bit
    } &  1    \\
        \textbf{4-bit
    } &  0.5    \\
    \bottomrule
    \end{tabular}
    \label{tab:best_combination}
    % \vskip -0.2in
\end{table}


==> tables/energy_analysis.tex <==
\begin{figure*}[t!]
    \begin{minipage}{0.5\textwidth}
    \begin{table}[H]
      \centering
    %   \vskip -0.1in
      \caption{Energy efficiency per training iteration (Datapath unit only)}
    %   \vskip 0.05in
    % \tabcolsep=0.09cm
    \small
    \begin{tabular}{cccc}
        \toprule
        \textbf{Model} & 
        \begin{tabular}{@{}c@{}}\textbf{LNS}\\(mJ)\end{tabular} &
        \begin{tabular}{@{}c@{}}\textbf{INT8}\\(mJ)\end{tabular} &
        \begin{tabular}{@{}c@{}}\textbf{FP16}\\(mJ)\end{tabular} \\
        \midrule
        %Energy Efficiency (images/s/W)  & 4489 & 6438 & 7124 \\
        \textbf{ResNet-18} & 0.15 & 0.23 & 3.34 \\
        \textbf{ResNet-50} & 0.28 & 0.42 & 6.15 \\
        \textbf{BERT-Large} & 8.12 & 11.98 & 173.73 \\
        \bottomrule
        
      \end{tabular}
    %   \vskip -0.25in
      \label{tab:energy_analysis}
    \end{table}
    \end{minipage}
\end{figure*}


==> tables/glue_results.tex <==
\begin{table}[h!]
  \centering
\begin{tabular}{lccc}
    \toprule
    \textbf{Tasks} & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    \textbf{MRPC (Accuracy \%)} & & & \\
    Base-2 Madam & \textbf{81.4} & \textbf{82.7} & \textbf{89.3} \\
    LogQuant     & 72.6 & 80.9 & 88.5  \\
    & & & \\
    \textbf{QNLI (Accuracy \%)} & & & \\
    Base-2 Madam & \textbf{57.6} & 59.5 & \textbf{89.6} \\
    LogQuant     & 51.2 & \textbf{78.5} & 89.4  \\
    %& & & \\
    %\textbf{QQP (Accuracy \%)} & & & \\
    %Base-2 Madam &  &  &  \\
    %LogQuant     &  &  &   \\
    %& & & \\
    \bottomrule
    
  \end{tabular}
  \caption{Benchmark on GLUE. }
  \label{tab:glue_results}
\end{table}





==> tables/imagenet_compare.tex <==
% left

==> tables/imagenet_results.tex <==
\begin{table}[h!]
  \caption{Benchmark on Image Classification}
  \centering
\begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{3}{c}{\textbf{ImageNet}} & \multicolumn{3}{c}{\textbf{CIFAR-10}} \\
    \textbf{Method} & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} &
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    Base-2 Madam  & 61.5 & 65.8 & 69.7 & & & \\
    Base-2 Madam (SGD warmup) & 64.8 & 67.7 & 71.9 & & & \\
    LogQuant & 67.1 & 69.4 & 73.6 & & & \\
    %Base-2 Madam (sign) & & & 69.8 & & & \\
    \bottomrule
    
  \end{tabular}
  \label{tab:image_results}
\end{table}




==> tables/squad_results.tex <==
\begin{table}[h!]
  \centering
\begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{3}{c}{\textbf{BERT}} & \multicolumn{3}{c}{\textbf{BERT-Large}} \\
    \textbf{Method} & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} &
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    \textbf{Low-Precision Training} & & & & & & \\
    Base-2 Madam (default parameters) & 3.7 & 80.6 & 87.9 & 3.9 & 82.6 & 89.3 \\
    Base-2 Madam & \textbf{11.2} & \textbf{84.1} & \textbf{88.0} & \textbf{13.8} & \textbf{86.0} & \textbf{90.3} \\
    LogQuant &  1.9 &  7.2 &  80.0 & 1.9 & 7.5 & 88.6 \\
    & & & & & & \\
    \textbf{Post-Training Quantization} & & & & & & \\
    UniformQuant & 2.2 & 7.3 & 64.3 & 2.4 & 9.0 & 88.6 \\
    \bottomrule
    
  \end{tabular}
  \caption{Benchmark on SQuAD. We fine-tune both BERT and BERT-Large on SQuAD and compute the F1 score. Default parameters mean that we apply the same integer step size $\eta^{*}$ and calibration method as the settings on ImageNet training. LogQuant represents low-precision using logarithmic representation with default AdamW optimzer. UniformQuant is a standard scaled quantization that applies to a well-trained model. For the reference, full-precision state-of-the-art results for BERT and BERT-Large model are 84.2 and 90.9, respectively. }
  \label{tab:squad_results}
\end{table}





==> tables/squad_results_exact_score.tex <==
\begin{table}[h!]
  \caption{Benchmark on SQuAD}
  \centering
\begin{tabular}{ccccccc}
    \toprule
    & \multicolumn{3}{c}{\textbf{Base-BERT}} & \multicolumn{3}{c}{\textbf{Large-BERT}} \\
    \textbf{Method} & 
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} &
    \textbf{4-bit} &
    \textbf{6-bit} &
    \textbf{8-bit} \\
    \midrule
    \textbf{Low-Precision Training} & & & & & & \\
    Base-2 Madam (default parameter) & 0.4/3.7 & 71.3/80.6 & 80.3/87.9 & 0.6/3.9 & 73.3/82.6 & 81.9/89.3 \\
    Base-2 Madam & 5.1/11.2 & 75.7/84.1 & 80.6/88.0 & 7.2/13.8 & 78.1/86.0 & 83.6/90.3 \\
    LogQuant &  0.6/1.9 &  1.3/7.2 &  70.1/80.0 & 0.7/1.9 & 1.3/7.5 & 80.7/88.6 \\
    & & & & & & \\
    \textbf{Post-Training Quantization} & & & & & & \\
    UniformQuant 0.1/0.1 & 0.2/7.2 & 52.2/64.3 & & & & \\
    \bottomrule
    
  \end{tabular}
  \label{tab:language_results}
\end{table}

==> tables/various_bitwidth.tex <==
\begin{table}[H]
\caption{\small{Unified bitwidth setting for $\bitwidth_{W}$, $\bitwidth_{A}$ and $\bitwidth_{E}$ on ImageNet. The combinations of $\bitwidth$ and $\gamma$ follow a fixed log dynamic range selected in Table \ref{tab:base_factor_selection}. We compare LNS and INT with different scaling techniques.  The results of test accuracy (\%) are shown below. }}
\centering
\small
\tabcolsep=0.15cm
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Bitwidth $\bitwidth$} & \textbf{Base Factor $\gamma$} & \textbf{LNS (per-vector)} & \textbf{LNS (per-layer)} & \textbf{INT (per-vector)} & \textbf{INT (per-layer)}
    \\
    \midrule
        \textbf{8-bit
    } & 8 &  76.05 & 75.96 & 75.69 & 75.30  \\
        \textbf{7-bit
    } & 4 &  76.10 & 76.24 & 75.01 & 72.65   \\
        \textbf{6-bit
    } & 2 &  75.83 & 75.83 & 74.25 & 65.20   \\
        \textbf{5-bit
    } & 1 &  75.55 & 75.13 & 73.59 & 43.97   \\
    %     \textbf{4-bit
    % } & 0.5 &  \text{NaN} & 70.96 & \text{NaN} & \text{NaN}  \\
    \bottomrule
    \end{tabular}
    \label{tab:various_bitwidth}
    % \vskip -0.2in
\end{table}

